RAAD-LLM: Adaptive Anomaly Detection Using LLMs and RAG Integration

Anomaly detection in complex industrial environments poses unique challenges, particularly in contexts characterized by data sparsity and evolving operational conditions. Predictive maintenance (PdM) in such settings demands methodologies that are adaptive, transferable, and capable of integrating domain-specific knowledge. In this paper, we present RAAD-LLM, a novel framework for adaptive anomaly detection, leveraging large language models (LLMs) integrated with Retrieval-Augmented Generation (RAG). This approach addresses the aforementioned PdM challenges. By effectively utilizing domain-specific knowledge, RAAD-LLM enhances the detection of anomalies in time series data without requiring fine-tuning on specific datasets. The framework's adaptability mechanism enables it to adjust its understanding of normal operating conditions dynamically, thus increasing detection accuracy. We validate this methodology through a real-world application for a plastics manufacturing plant and the Skoltech Anomaly Benchmark (SKAB). Results show significant improvements over our previous model with an accuracy increase from 70.7% to 88.6% on the real-world dataset. By allowing for the enriching of input series data with semantics, RAAD-LLM incorporates multimodal capabilities that facilitate more collaborative decision-making between the model and plant operators. Overall, our findings support RAAD-LLM's ability to revolutionize anomaly detection methodologies in PdM, potentially leading to a paradigm shift in how anomaly detection is implemented across various industries.

==> component_subject_sections/Background/background-not-used.tex <==
\subsection{Fundamental Concepts and Terminology}

This section serves as a background for understanding LLMs and adaptive anomaly detection as presented in this paper. It aims to provide key terms, baseline definitions, and relevant mathematical notations that are essential for comprehending the concepts discussed. Additionally, this section briefly discusses the initial stages of our research endeavor. It describes the preliminary investigations conducted to lay the groundwork for our current work.

A \textbf{large language model (LLM)} is trained on sequences of tokens and encodes an auto-regressive distribution, where the probability of each token depends on the preceding ones \cite{LLM_zero_shot_TS}. More simply, an LLM is trained on sequences of words or word pieces, and the output is the likelihood of the next word in a sequence given the previous words (i.e., context-aware embeddings). Each model includes a tokenizer that converts input strings into token sequences. Models like GPT-3 and LLaMA-2 can perform zero-shot generalization, effectively handling tasks without specific training  \cite{LLM_zero_shot_TS}. For this work, we repurpose an LLM for time series anomaly detection while keeping the backbone language model intact \cite{Time_LLM}. A binarization function is then applied to the outputs of the LLM to map them to $\{0,1\}$ to obtain the final predictions. The exact binarization function is use-case specific.

\textbf{Transfer learning} is a machine learning technique where the knowledge gained through one task is applied to a related task  with low/no retraining \cite{10.5555/1803899}. Specifically, in transfer learning, we train a model to perform a specific task on the source domain and then make certain modifications to give us good predictions for a related task on the target domain where data is (usually) scarce or a fast training is needed \cite{Neyshabur2020WhatIB}. For this work, we leverage a pretrained LLMs' text synthesizing and reasoning abilities acquired through training on a source domain by transferring this task knowledge to our PdM use-case. Specifically, we show that pretrained LLMs can effectively predict anomalies in time series data by transferring its text synthesizing and reasoning knowledge to our target manufacturing domain. 

\textbf{Concept drift} is the phenomenon where the statistical properties of a domain changes over time, which can then result in a deterioration of models that have previously been trained within that domain \cite{Stachl2019RepositoryPR, BERGGREN2024112465}. In particular, it can lead to a degradation of performance of static models as they become less effective in detecting anomalies.  For example, in manufacturing, the statistical properties of raw material attributes change over time. Therefore, if these variables are used as product quality predictors, the resulting models may decrease in validity. 

\textbf{Adaptive anomaly detection (AAD)} encompasses techniques that can detect anomalies in data streams or in situations where concept drift is present. These techniques make models capable of automatically adjusting their detection behavior to changing conditions in the deployment environment or system configuration while still accurately recognizing anomalies \cite{Steenwinckel2021FLAGSAM, Steenwinckel2018AdaptiveAD}. For this work, the \textbf{adaptability mechanism} refers to the feature that enables the model's definition of normality and related statistical derivatives to adjust with each new data instance. 

\textbf{Windowing} refers to dividing a time series into smaller, manageable segments, which are then processed individually. Windowing (or \textit{sliding window technique}) is used extensively for anomaly detection in time series data due to its many benefits \cite{w13131862}. For our use-case, dividing the time series into windows helps to preserve local information that might be lost when considering the entire time series as a whole and reduce computational load since models can handle smaller inputs more efficiently.  

A process is said to be \textit{"in statistical control"} if it is not experiencing out of control signals or significant variations beyond normal statistical variations \cite{mcshane2023asq}. \textbf{Statistical process control (SPC)} techniques are commonly used in manufacturing for monitoring sequential processes (e.g., production lines) to make sure that they work stably and satisfactorily \cite{Qiu2018SomePO}. In monitoring the stability of a process, statistical process monitoring (i.e., SPC) plays an essential role \cite{qiu2013introduction, SONG2023109469}. The idea is that processes that are in statistical control are deemed to be \textit{stable} processes \cite{mcshane2023asq}. For this work, stable processes form a baseline for \textbf{normal} process behavior. The selection of SPC techniques are use-case specific. For this work, MAMR is implemented. \textbf{Moving average moving range (MAMR)} charts are plotted for each process variable in the time series dataset as shown in \autoref{fig:fig_meth3}. Upper (UCL) and lower (LCL) control limits for the moving average ($X$) and moving range ($mR$) charts are calculated as follows.

\setlength\parindent{50pt} $X$ Chart:
\begin{equation} \label{eq:xucl}
UCL = \overline{X} + 2.66\overline{R}
\end{equation}

\begin{equation} \label{eq:xlcl}
LCL = \overline{X} - 2.66\overline{R}
\end{equation}

$mR$ Chart:
\begin{equation} \label{eq:rucl}
UCL= 3.27\overline{R}
\end{equation}

\setlength\parindent{14pt} %reset indentation amount
The values $2.66$ and $3.27$ are often used as multipliers for estimating control limits in the MAMR chart. However, these multipliers can significantly widen the control limits, making them less sensitive to minor shifts or variations in the process. Therefore, it is important to analyze historical data to determine the typical variability in the process under consideration and select multipliers that reflect the process's actual behavior while maintaining sensitivity.

\subsection{Investigated Approaches in Expert Systems for PdM}

Through a thorough review of existing literature, initial data collection, and exploratory data analysis, we aimed to gain insights into the complexities of anomaly detection for PdM and to establish a basis for our subsequent research inquiries. This preliminary work allowed us to uncover initial patterns, trends, and areas of interest, shaping the development of our research framework and guiding the formulation of our research hypothesis for the current work.

A case study conducted for a leading plastics manufacturing plant highlighted the use of anomaly detection algorithms for predictive maintenance (PdM) to analyze failures in the plastics extrusion process. An overview of the plastics extrusion process can be seen in \autoref{fig:fig_process}. By identifying and correlating anomalies with other process variables, operators can uncover root causes of failures. This would allow for targeted corrective actions and improved predictions of future failures.

\begin{figure}
    \includegraphics[width=0.45\textwidth]{images/process.png}
    \caption{Process flow diagram of major components in our use-case extrusion process. The major components in the extrusion process are in a series configuration. The number of Feed and Screw/Barrel Systems depends on the manufacturing line number and can be 3, 4, or 5.}
    \label{fig:fig_process}
\end{figure}

Our investigation focused on screen pack failures since shutdowns due to these failures were well documented in the data. An example of a screen pack changer can be seen in \autoref{fig:fig_screenpack}. For two downtime events with screen pack failure mode, we obtained 65 hours of historical run-to-failure sensor readings. The readings were semi-labeled and for process variables that were deemed good indicators of screen pack failures. These process variables are as follows and for any of these, sudden spikes from expected profile could signal significant process variable deviations; and therefore, could lead to a screen pack failure.

\begin{itemize}
    \item \textit{Melt Pressure 1} is the melt viscosity at the screen inlet. 
    \item \textit{Temperature 1} is the melt temperature at the screen pack inlet. 
    \item \textit{Melt Pressure Differential} is the melt pressure across the screen pack inlet and outlet. 
\end{itemize}

\begin{figure}
    \includegraphics[width=0.5\textwidth]{images/screenpack3d.png}
    \caption{The die head system for our use-case. The screen pack changer is identified by a red box. Within the screen pack changer, screen packs are used to prevent impurities from getting into the extruder together with the resin and thus clogging the die gap. The number of screen packs depend on the number of Screw/Barrel Systems. Each screen pack is arranged between the Screw/Barrel System and the Die Head System. During production, the resin melts flow through the screen pack.}
    \label{fig:fig_screenpack}
\end{figure}

The data, however, was scarce and noisy; and therefore, presented many challenges in its analysis. Maintenance logs identified shutdown couses, but lacked details on failures' location and timing. Understanding failures requires synthesizing this information to uncover root causes and systemic issues. Moreover, the absence of a baseline for normal process behavior further complicated analysis. The variability in statistical characteristics across processes was influenced by product mix, component age, wear, and component type heterogeneity.

For the PdM use case, we effectively employed anomaly detection techniques to overcome challenges by integrating domain knowledge, expert rules, sensor readings, and maintenance logs. We developed a statistics-based predictive model using SPC techniques to establish control limits, then applied dynamic time warping (DTW) for anomaly detection in time-series data. Anomalous distances were identified through the Mann-Whitney U test, and an adaptability mechanism improved detection accuracy by allowing the model to adjust to evolving conditions. With $83.3\%$ accuracy, the methodology demonstrated the feasibility of anomaly detection for PdM in complex, dynamic, and data-constrained industrial settings. It also highlighted the potential for substantial cost savings, minimized downtime, and enhanced asset reliability. 

However, this initial approach lacked transferability and multimodality. The statistics-based model relied on domain-specific rules and knowledge to perform well. Domain-specific knowledge (e.g. process parameter optimal ranges, equipment specifications, etc.) cannot usually be applied across domains and therefore would limit model application across diverse industrial settings. Furthermore, the absence of multimodality hindered fusion of diverse input sources (e.g., series data and maintenance logs) for synergistic forecasting. This limitation prevented the enrichment of input sensor readings with semantics. Consequently, domain expertise had to be manually translated into the computational model; therefore impeding collaborative decision-making between the model and plant operators.

Adaptive anomaly detection using large language models (AAD-LLM) was developed as a novel framework that repurposed LLMs for anomaly detection within manufacturing time series data. Since the model doesn't require any training or finetuning on the data set it is applied to, it was shown to improve transferability in data-constrained contexts. Additionally, the framework was shown to enable the enrichment of input time series data with semantics to deliver more collaborative decision-making between the model and plant operators. Lastly, an adaptability mechanism similar to that used for the statistics-based approach was leveraged to enhance detection accuracy.

For the use-case dataset, the model achieved an accuracy of $70.7\%$. The outcomes of this work presented compelling insights into the potential and effectiveness of LLMs for anomaly detection tasks, specifically for the PdM use-case. These findings highlighted the model’s capacity to detect anomalies within time series data effectively; even in complex and dynamic operational settings. Although preliminary results were good, the LLM was not consistent in correctly making comparisons between current and normal operating statistical derivatives. These comparisons are critical for effective anomaly detection. 

We hypothesize that the performance of AAD-LLM can be improved by integrating a full RAG pipeline into the architecture. Specifically, RAG would aid the model in performing number comparisons and math calculations. Preliminary findings indicated that the inability of the current model to do these things consistently, reduced its overall performance. 

With RAG, LLMs can potentially learn to interpret and solve math problems stated in natural language. By leveraging the capabilities of a RAG along with the inherent language understanding and reasoning abilities of the LLM, AAD-LLM can be adapted to handle mathematical tasks effectively. This new architecture is referred to as RAAD-LLM. The improved performance of RAAD-LLM will emphasize LLMs capability and promise in excelling in time series anomaly detection tasks; even in data-constrained industrial applications. Therefore, the proposed work will contribute significantly to advancements in anomaly detection methodologies.

==> component_subject_sections/Conclusion/conclusion-nout_used.tex <==
In the RAAD-LLM framework, the availability of domain-specific knowledge is effectively harnessed to optimize the capabilities of LLMs for anomaly detection tasks. Incorporating the RAG component improves model performance, thus facilitating greater collaboration between the model and plant operators in decision-making processes. Furthermore, the adaptability mechanism enables the model to continuously refine its understanding of normal behavior in response to shifts in system operational conditions over time. Consequently, RAAD-LLM maintains an up-to-date perspective of normal system behavior to make accurate predictions despite the dynamic nature of operational settings. By utilizing SPC techniques to establish the baseline, this methodology eliminates the need for the model to \textquote{learn} normal behavior. Therefore, the model maintains high transferability with zero-shot capabilities. The results indicate that anomaly detection can be effectively approached as a language task, delivering context-aware detection solutions that are particularly valuable in data-sparse industrial applications.

Although evaluation metrics demonstrate proof-of-concept, the model framework can be improved. The RAAD-LLM architecture requires that all domain context be added to the prompt before being fed through the frozen LLM. This made the query too complex, leading to inconsistent responses that often did not align with expectations. To address this issue, we manually restructured the \textquote{raw} domain context. This restructuring better guided the LLM's decision-making, but it took a lot of time and effort. RAAD-LLMv2 was designed to address this issue and be more scalable in real-world settings. However, it exhibited slightly lower performance compared to RAAD-LLM. Further work should explore fine-tuning LlamaIndex configurations or hybrid approaches that blend manual context restructuring with automated retrieval. Lastly, RAAD-LLM was applied to only static datasets to better understand how processes failed after the failure had already occurred. However, further work should explore the extension of the methodology to data streams for online anomaly detection.


==> component_subject_sections/Methodology/methodology-original.tex <==
This section overviews the RAAD-LLM methodology and outlines the proposed enhancement of the AAD-LLM framework through the incorporation of a RAG pipeline. The goal of this enhancement is to improve the model’s capacity to perform complex reasoning tasks that require computational support. The integration of the RAG pipeline into the AAD-LLM framework allows the model to access external knowledge bases dynamically and incorporate relevant information into its decision-making process. This combination enhances the LLM's performance in recognizing and classifying anomalies. As a result, this integration will strengthen RAAD-LLM's ability to detect anomalies in data-sparse industrial environments.

\subsection{The RAAD-LLM Framework}

The following subsections provide a detailed description of the RAAD-LLM architecture as shown in \autoref{fig:fig_meth1}. It discusses the key components, domain-specific knowledge integration, data processing workflow, and the methodology for combining prompting, RAG, and model inference to enhance anomaly detection capabilities.

\subsubsection{System Architecture}

The integrated architecture, referred to as RAAD-LLM, consists of the following key components:
\begin{enumerate}
\item \textit{Pretrained LLM:} A pretrained LLM serves as the foundation model for anomaly detection. For this work, Meta Llama 3.1 8B model was chosen since it is an open source instruction-fine-tuned LLM demonstrating state-of-the-art on tasks such as classification, question answering, extraction, reasoning, and summarizing \cite{Zhang2023InstructionTF}. This model remains frozen during processing to maintain transferability.
\item \textit{RAG Component:} The RAG component incorporates a CSV-based knowledge base that dynamically retrieves contextually relevant information for z-score comparisons. This functionality enables the model to provide responses reflecting either exact matches for input values or the closest available matches when exact values are not found. Consequently, the integration of RAG improves both the accuracy and interpretability of sensor data queries.
\item \textit{Anomaly Detection Layer:} For each time series window under consideration, this layer applies SPC techniques and the Discrete Fourier Transform (DFT), and then computes historical and current statistical measures. Next, utilizing domain-specific knowledge, text templates, and a binarization function anomaly classification is performed.
\item \textit{Adaptability Mechanism:} This feature continuously updates the baseline normal behavior as each new time series window is processed. 
\end{enumerate}

The LLM hosting environment is built around Ollama, which supports the Llama 3.1 8b model. This server acts as the central endpoint for processing context-aware prompts. The server’s base URL is specified, and parameters like request timeout and maximum tokens are configured to ensure steady communication and manage resource usage.

\subsubsection{Domain-Specific Knowledge and Text Templates}

To enhance collaboration with plant operators, we develop a domain-specific context file that enables the LLM to comprehend the specifics of our time series data. This file integrates expert rules, domain knowledge, and constraints to establish acceptable ranges for process variable variations, guide feature selection, and describe in detail causal relationships among variables. In our manufacturing use case, comprising 580 sensors per line, operators can correlate these readings with failure modes. Furthermore, fluctuations in raw materials necessitate adjustments in process parameters, which polymer scientists can specify. By utilizing this expertise, we can refine thresholds, select relevant features, and identify interactions; thereby improving anomaly detection. The context file is imported and should be persisted for efficiency. 

To enable structured understanding and improved performance, we create text templates with placeholders that align with essential statistical values such as mean, standard deviation, and maximum. In this work, only the z-score is used, as prior research found it sufficient to yield good results. When actual data is available, these placeholders are populated through data injection. Injected statistical measures for both normal system behavior and the current query window under consideration will guide the LLM’s reasoning, enhancing its anomaly detection capabilities.

%begin textbox
\begin{center}
    \begin{minipage}{9cm}            
        \begin{tcolorbox}[enhanced,attach boxed title to top center={yshift=-1mm,yshifttext=-1mm},
                colback=green!10!white,colframe=gray!90!black,colbacktitle=gray!80!black, left=0.1mm, right=0.5mm, boxrule=0.50pt]
        %TEXT                
        \textbf{INSTRUCTIONS:} You are a helpful assistant that can use these rules to answer queries. The following sensor data was collected over the last 15 minutes and represent current process conditions. Strictly based on the context and RAG information provided below, please answer the following questions. Do not modify, interpret, or apply logic beyond these instructions. \\ 
        * Is high deviation present for Melt Pressure 1? \\
        * Is high deviation present for Melt Pressure Differential? \\
        For each question, avoid explaining. Just print only the output and nothing else. \\        
        \textbf{CONTEXT:} \textcolor{red}{$<$cached info$>$} \\
        \textbf{DATA:} Melt Pressure 1 has a z-score of \textcolor{red}{$<$val$>$}. Melt Pressure Differential has a z-score of \textcolor{red}{$<$val$>$}. \\
        \textbf{RAG:} The z-score for Melt Pressure 1 is \textcolor{red}{$<$greater than / less than / equal to$>$} acceptable process variable conditions. The z-score for Melt Pressure Differential is \textcolor{red}{$<$greater than / less than / equal to$>$} acceptable process variable conditions.

        \end{tcolorbox}
    \end{minipage}
\end{center}
\vspace{0mm}
\captionof{figure}{Prompt example. \textcolor{red}{$<$cached info$>$} is the domain context information. \textcolor{red}{$<$val$>$} are calculated statistical measures injected into respective text templates. \textcolor{red}{$<$greater than / less than / equal to$>$} is the relevant z-score comparison information from the RAG retriever. Note that although each $Q_i$ is processed independently, prompts include text templates for all $i \in N$ where $N$ is the number of input variables in instance $Q$ from the dataset $D$ under consideration. Therefore, multivariate anomaly detection is explored. }\label{fig:prompt_text}
\vspace{4mm}
%end textbox

\setlength\parindent{12pt}
\subsubsection{Data Processing Workflow}

Defining normal process behavior is crucial for effective anomaly detection, as it establishes a baseline against which potential anomalies can be compared and identified. This baseline is determined in a manner akin to the AAD-LLM methodology. From the dataset D under consideration, a multivariate time series instance $Q\in \mathbb{R}^{N\times T}$ is partitioned into $N$ univariate time series where $N$ is the number of input variables and $T$ is the number of time steps. This is done so that each input variable is processed independently \cite{Time_LLM}. 

Each $i^{th}$ series $Q_i, i \in N$, is then processed using SPC techniques as shown in \autoref{fig:fig_meth3}. Time series points deemed \textquote{out of statistical control} are labeled as anomalous and filtered out of $Q_i$ before further processing. SPC is applied again after the first set of outliers (or anomalies) are removed. This is done to ensure extreme values do not affect control limits. 

Unlike, AAD-LLM, MEWMA is applied as a phase II SPC implementation to further refine MAMR control limits. Therefore, it can be assumed that time series $Q_i$ represents a stable process. We use this assumption in initializing our comparison dataset $C_i$ as our baseline for normal behavior as explained in the next paragraph. The idea is that once the comparison dataset is initialized, the model then updates its understanding of normalcy as each new query window is ingested.

Rather than processing the entire time series at once, $Q_i$ then undergoes windowing as shown in \autoref{fig:fig_meth1}. For each $i \in N$, windowing divides time series $Q_i$ into $P$ consecutive non-overlapping segments of length $L$, $Q_i^{(P)} \in \mathbb{R}^{P \times L}$. By analyzing data within sliding windows, anomaly detection can focus on smaller segments of the time series data. This provides a more granular and detailed view of abnormal patterns. Processing the entire time series as a single entity might obscure localized anomalies within the data. Finally, for each $i \in N$, a baseline dataset $C_i \in \mathbb{R}^{1 \times L}$ of normal behavior is defined as the first $Q_i$ window.  

Unlike AAD-LLM, for each $i \in N$, both the current $Q_i$ window $Q_i^{(p)}$ where $p \in P$ and the baseline data set, $C_{i}$ undergo additional processing through the DFT. Since sensor signals are sampled discretely, the DFT is very useful in their analyses \cite{e2019troubleshooting}. Specifically, the DFT can be used to isolate the most prominent frequency component from the noise, thereby enhancing the discernibility of the signal. After applying the DFT, we then construct a sinusoidal representation of the dominant frequency component for both $ Q_i^{(p)} $ and $ C_i $. The steps to apply the DFT and then construct a sinusoidal representation are as follows.

The DFT for signal $s(t)$ is computed as:
\begin{equation}
    F(k) = \sum_{t=0}^{N-1} s(t) \cdot e^{-i \cdot 2\pi \frac{k \cdot t}{N}} \quad \text{for } k = 0, 1, \dots, \frac{N}{2}
\end{equation}
Here, $F(k)$ represents the frequency components, with the focus on the real part of the spectrum.

The amplitude spectrum is computed as the scaled magnitude of the Fourier coefficients:
\begin{equation}
A_k = \frac{2}{N} \left| F_k \right| \quad \text{for } k = 0, 1, \dots, \frac{N}{2}
\end{equation}
where:
\begin{itemize}
    \item $A_k$ is the amplitude corresponding to the $k$-th frequency component,
    \item $F_k$ is the $k$-th Fourier coefficient from the DFT output.
\end{itemize}

The dominant frequency and amplitude are determined as:
\begin{equation}
f_{\text{max}} = f_k \quad \text{where } k = \arg\max_k A_k
\end{equation}

\begin{equation}
A_{\text{max}} = A_k \quad \text{for the same } k
\end{equation}
where:
\begin{itemize}
    \item $f_{\text{max}}$ is the dominant frequency in the signal,
    \item $A_{\text{max}}$ is the amplitude of the dominant frequency.
\end{itemize}

Using $f_{\text{max}}$ and $A_{\text{max}}$, a sine wave is fitted to represent the dominant signal component:
$$
\hat{s}(t) = A_{\text{max}} \cdot \sin(2 \pi f_{\text{max}} \cdot t) + \left| \bar{s} \right|
$$
where:
\begin{itemize}
    \item $\hat{s}(t)$ is the reconstructed sine wave signal,
    \item $A_{\text{max}}$ is the amplitude of the dominant frequency,
    \item $f_{\text{max}}$ is the dominant frequency,
    \item $\bar{s}$ is the mean value of the original signal that is added to account for offset adjustments,
    \item $t$ represents time.
\end{itemize}

Subsequently, selected statistical measures for the sinusoidal representations of $Q_i^{(p)}$ and $C_i$ are calculated and then injected into the corresponding text templates. This approach is advantageous because it allows for a clearer differentiation between signal and noise, making it easier to identify patterns and anomalies in the data. By focusing on frequency components, we gain a deeper understanding of the underlying dynamics of the signal.

\subsubsection{Prompting, RAG, and Model Inference} \label{sec:prompting}

Prompts are then created via prompt engineering and combined with the templates. To further enrich the inputs, the domain context is added to the prompt before being fed forward through the frozen LLM. For our methodology, the domain context was manually restructured from the \textquote{raw} domain context to reduce the complexity of the input prompt. Consequently, this better guided the LLM's decision making, thereby enabling more consistent predictions. Effective prompt engineering is essential in ensuring accurate, context-aware anomaly detection.

Prior to predicting anomalies, the statistical measures for all input variables are sent to the RAG component to retrieve relevant z-score comparison information from the knowledge base. The retrieved information is then combined with the prompt, allowing the LLM to better understand the relationship between the historical normal and the observed statistics of the process being monitored. A prompt example is shown in \autoref{fig:prompt_text}. The resultant enriched prompt is fed forward through the frozen LLM. 

%begin textbox
\begin{center}
    \begin{minipage}{9cm}            
        \begin{tcolorbox}[enhanced,attach boxed title to top center={yshift=-1mm,yshifttext=-1mm},
                colback=green!10!white,colframe=gray!90!black,colbacktitle=gray!80!black, left=0.1mm, right=0.5mm, boxrule=0.50pt]
        %TEXT                
        * High deviation present for Melt Pressure 1. \\
        * High deviation is not present for Melt Pressure Differential.    

        \end{tcolorbox}
    \end{minipage}
\end{center}
\vspace{0mm}
\captionof{figure}{LLM output example. Outputs are an itemized list of process variables and their anomaly status. The text-based outputs use domain-specific terminology, enabling subject matter experts to interpret findings more easily than numerical results and fostering better collaboration and knowledge transfer.}\label{fig:llm_output}
\vspace{4mm}
%end textbox

\setlength\parindent{12pt}
An example output of the LLM is shown in \autoref{fig:llm_output}. The LLM outputs an itemized list indicating whether an anomaly is present for each process variable. The textual outputs of the LLM enhance collaboration with subject matter experts because they are more accessible and easier to interpret than purely numerical results. These text-based outputs incorporate domain-specific terminology that allow experts to understand findings without the need to decode complex numbers. This enhancement fosters better communication and feedback loops between technical and non-technical team members. Consequently, experts can validate or challenge the model’s conclusions more effectively. Ultimately, this approach promotes improved knowledge transfer and bridges the gap between expert systems and domain expertise, making the outputs significantly more actionable and user-friendly.

Lastly, we apply a binarization function to the LLM's outputs to map them to $\{0,1\}$ to get the final classification ($0=$ non-anomalous, $1=$ anomalous). The exact binarization function is use-case specific. For our use-case, one anomaly alone does not sufficiently indicate a problem. To avoid false positives that trigger an unnecessary shutdown, our binarization function only maps to $1$ if anomalies in the output are correlated as indicated by domain-specific knowledge. Let $x$ be the LLM output. Then

\begin{equation}
%\[
     f(x) =
    \begin{cases} 
        1, & \text{if anomalies in } x \text{ are correlated} \\
        0, & \text{otherwise}
     \end{cases}
%\]
\end{equation}

The final classification is what is used for determining updates to $C_i$ before moving to the next $Q_i^{\left(p\right)}$. If the output prediction indicates no anomalies in $Q_i^{\left(p\right)}$, window $Q_i^{\left(p\right)}$ series data is combined with the preceding windows series data to gradually refine the dataset of what constitutes \textquote{normal} behavior $C_i$. Therefore, for each $i \in N$, $C_i$ is guaranteed to be representative of normal behavior and is constantly evolving.


\subsubsection{Adaptability Mechanism}

The adaptability mechanism of AAD-LLM is preserved in the RAAD-LLM framework. In addition to $C_i$ constantly updating as each new query window is ingested, the process of re-initializing $C_i$ is done for each new instance $Q$. This continuous redefining of the normal baseline enables the model to progressively refine its knowledge in response to shifts in the system’s operational conditions process after process. Therefore, the model is enabled to maintain an up-to-date and broad perspective of normality. 

\begin{table*}[!t]
    \begin{center}
    \begin{tabular}{| c | c |}
    \hline
    \textbf{Component} & \textbf{Details} \\
    \hline
    \hline
    LLM Model &  Meta Llama 3.1 model (8B parameters) \\
    \hline
    Server Base URL & Hosted on a private network at http://localhost:11434 \\
    \hline
    Request Timeout & 500 seconds \\
    \hline
    Output Temperature & 0.2 \\
    \hline
    Token Limit & 250 tokens \\
    \hline
    Mirostat & Disabled (mirostat: 0), ensuring deterministic output generation \\
    \hline
    Embedding Use & The LLM is utilized to generate embeddings for domain-specific vector stores for efficient context retrieval. \\
    \hline
    \end{tabular}
    \caption{Configuration summary table of the LlamaIndex and Ollama system. This setup facilitates seamless retrieval of relevant domain knowledge from the vector store using LlamaIndex. Rather than all the domain context, only the retrieved content is added to the prompt before being fed forward through the frozen LLM.} 
    \label{table:config}
    \end{center}
\end{table*}


\begin{figure}
    \includegraphics[width=0.48\textwidth]{images/llamaindex.png}
    \caption{The LlamaIndex flowchart representation.  Raw domain context information is loaded as input. Each data chunk is processed using an embedding model (in this case, LLama 3.1 8b from the Ollama server). Parameters such as temperature (0.2), max tokens (250), and mirostat (disabled) are set to ensure robust and consistent embeddings are generated for the context. The generated embeddings are then stored as vectors in a vector database. Finally, LlamaIndex structures the database by organizing and indexing the embeddings into a retrievable format. The vector store then becomes accessible to the RAG component, allowing dynamic retrieval of relevant domain context as needed.}
    \label{fig:fig_llamaindex}
\end{figure}

\subsection{The RAAD-LLMv2 Framework with LlamaIndex Integration}

The RAAD-LLM architecture requires that all domain context be added to the prompt before being fed through the frozen LLM. This made the query too complex, leading to inconsistent responses that often did not align with expectations. To address this issue, we manually restructured the \textquote{raw} domain context as described in Section \ref{sec:prompting}. This restructuring better guided the LLM's decision-making, but it took a lot of time and effort.

The RAAD-LLMv2 variant extends RAAD-LLM by integrating an additional RAG module powered by LlamaIndex.  LlamaIndex is open-sourced and has been proposed as a method to expand the context capabilities of LLMs by enabling them to utilize extensive documents and databases during response generation \cite{zirnstein2023extended, malviya2024scalability, malviyanew}. The new architecture dynamically retrieves relevant domain context rather than incorporating all the provided context into the prompt. Consequently, this new architecture enhances the model's decision-making by providing more accurate and consistent responses without manual context restructuring. Additionally, it is more scalable under real-world scenarios. \autoref{fig:fig_llamaindex} is a visual representation of the LlamaIndex process.

\subsubsection{LlamaIndex and Ollama System Configuration}

The configuration of the LlamaIndex and Ollama system is designed to enable effective interaction between the RAG component and the LLM for domain context retrieval and embedding generation. The following provides technical details about the integration, including the configuration of the LlamaIndex and Ollama system. 

\begin{enumerate}
\item \textit{Ollama LLM Server:} The LLM hosting environment is the same as for the RAAD-LLM framework. This server acts as the central endpoint for processing both context-aware prompts and embeddings for vector stores. 
\item \textit{Embedding Model:} The LlamaIndex relies on Ollama's embedding capabilities, using the same Llama 3.1 model as an embedding generator for the knowledge base. 
\item \textit{Parameter Tuning:} Both the LLM and embedding configurations include custom parameters optimized to balance accuracy and computational efficiency. These parameters govern model output behaviors, such as temperature (for controlling randomness), maximum token count (to limit the size of outputs), and the request timeout duration.
\end{enumerate}

Table \ref{table:config} details the LlamaIndex and Ollama system configuration used for this work. This configuration facilitates the retrieval of relevant information from a vector store to complement input prompts, thereby improving the LLM's contextual understanding.




==> component_subject_sections/Results/results-original.tex <==
This section discusses the analyses of the datasets and experimental outcomes of RAAD-LLM and RAAD-LLMv2. The focus is on their performance improvements and limitations when applied to anomaly detection tasks. These discussions aim to provide deeper insights into the frameworks' effectiveness and areas for future enhancement.

\subsection{Data and Analysis For the PdM Use-Case}

Our use-case dataset was for screen pack failures in the extrusion process since shutdowns due to these failures were well documented by the plastics manufacturing plant providing the data. An example of a screen pack changer can be seen in \autoref{fig:fig_screenpack} and an overview of the plastics extrusion process for our use-case can be seen in \autoref{fig:fig_process}. For two downtime events with screen pack failure mode, we obtained 65 hours of historical run-to-failure sensor readings (6.5 hours for 5 components for each downtime event). The readings were semi-labeled and for process variables that were deemed good indicators of screen pack failures. These process variables are \textit{Melt Pressure 1}, \textit{Temperature 1}, and \textit{Melt Pressure Differential}. 

\begin{figure}
    \includegraphics[width=0.45\textwidth]{images/process.png}
    \caption{Process flow diagram of major components in our use-case extrusion process. The major components in the extrusion process are in a series configuration. The number of Feed and Screw/Barrel Systems depends on the manufacturing line number and can be 3, 4, or 5.}
    \label{fig:fig_process}
\end{figure}

\begin{itemize}
\item Melt Pressure 1 - The melt viscosity at the screen inlet. 
\item Temperature 1 - The melt temperature at the screen pack inlet. 
\item Melt Pressure Differential - The melt pressure across the screen pack inlet and outlet. 
\end{itemize}
For any of these, sudden spikes from expected profile could signal significant process variable deviations; and therefore, could lead to a screen pack failure. Since \textit{Temperature 1} did not contain enough sample data, it was not selected as a feature. Therefore, only \textit{Melt Pressure 1} and \textit{Melt Pressure Differential} were input into RAAD-LLM and RAAD-LLMv2 for anomaly detection.

The domain context was meticulously collected from maintenance logs and plant operators. Maintenance logs provided detailed records of prior screen pack failures and anomalies. Additionally, plant operators contributed their expertise and firsthand knowledge, which helped define acceptable ranges for fluctuations and establish causal relationships among process variables. This collaborative approach ensured that the domain context effectively captured the operational intricacies of the manufacturing process.

\begin{figure}
    \includegraphics[width=0.5\textwidth]{images/screenpack3d.png}
    \caption{The die head system for our use-case. The screen pack changer is identified by a red box. Within the screen pack changer, screen packs are used to prevent impurities from getting into the extruder together with the resin and thus clogging the die gap. The number of screen packs depend on the number of Screw/Barrel Systems. Each screen pack is arranged between the Screw/Barrel System and the Die Head System. During production, the resin melts flow through the screen pack.}
    \label{fig:fig_screenpack}
\end{figure}

\begin{figure}
    \includegraphics[width=0.5\textwidth]{images/sensors.png}
    \caption{Processed sensor data from the SKAB dataset. The selected signals are preprocessed to include only those experiments that were 20 minutes in duration. Each signal begins in a non-anomalous experimental state and continues until the end of the experiment. Non-anomalous states are shown in \textcolor{blue}{blue} and anomalous states are shown in \textcolor{orange}{orange}. Processed signals are then input into the frameworks.}
    \label{fig:fig_sensors}
\end{figure}

\subsection{Data and Analysis For the SKAB Dataset}

The Skoltech Anomaly Benchmark (SKAB) is a publically accessible dataset designed for evaluating the performance of anomaly detection algorithms. The benchmark includes labeled signals captured by several sensors installed on the SKAB testbed. The SKAB testbed was specifically developed to study anomalies in a testbed. The focus of this work is to develop methods for detecting anomalies in these signals, which can be relevant for various applications. 

A description of the columns in the SKAB dataset is as follows \cite{skab}.
\begin{itemize}
    \item datetime - Dates and times when the value collected
    \item Accelerometer1RMS - Vibration acceleration (g units)
    \item Accelerometer2RMS - Vibration acceleration (g units)
    \item Current - The amperage on the electric motor (Ampere)
    \item Pressure - The pressure in the loop after the water pump (Bar)
    \item Temperature - The temperature of the engine body ($\degree C$)
    \item Thermocouple - The temperature of the fluid in the circulation loop ($\degree C$)
    \item Voltage - The voltage on the electric motor (Volt)
    \item RateRMS - The circulation flow rate of the fluid inside the loop (Liter per minute)
    \item anomaly - If the point is anomalous (0 or 1)
    \item changepoint - If the point is a changepoint (0 or 1)
\end{itemize}


The anomaly column contains the labels. A Mann–Whitney–Wilcoxon test (or Mann-Whitney U test) was used to determine whether any of the features in the dataset affected the labels. This test combined with a correlation matrix to detect relationships between variables resulted in \textit{Accelerometer1RMS}, \textit{Accelerometer2RMS}, \textit{Temperature}, and \textit{RateRMS} as selected features. Therefore, only these were input into RAAD-LLM and RAAD-LLMv2 to make the predictions. See \autoref{fig:fig_sensors} for further processing details.

Experiments on the SKAB dataset were conducted to determine the optimal fluctuation ranges for each of the selected features. The domain context file was determined without utilizing any prior domain knowledge. As a result, the context was built solely on a single statistical measure, which may have limited the accuracy of anomaly detection in this highly specialized system. Incorporating domain expertise could have enabled better feature selection, threshold setting, and understanding of variable interactions. Consequently, the model’s performance on the SKAB dataset may have been constrained, highlighting the potential for improvement through informed context creation. See Section \ref{sec: perf} for model performance on the SKAB dataset.

\subsection{Evaluation of Model Performance} \label{sec: perf}

\begin{table}[!h]
    \begin{center}
    Use-Case Dataset \\
    \begin{tabular}{| c | c | c | c | c |}
        \hline
        \textbf{Model} & \textbf{\shortstack{Accuracy \\ Baseline=0.709434}} & \textbf{Precision} & \textbf{Recall} & \textbf{F1 score}\\
        \hline
        \hline
        AAD-LLM & 0.706612 & 0.881481 & 0.683908 & 0.770227 \\
        \hline
        RAAD-LLM & 0.890566 & 0.966626 & 0.882051 & 0.922169 \\
        \hline
        RAAD-LLMv2 & 0.730817 & 0.964821 & 0.658120 & 0.782398 \\
        \hline
        \end{tabular}
        \bigskip
        
        SKAB Dataset \\
        \begin{tabular}{| c | c | c | c | c |}
        \hline
        \textbf{Model} & \textbf{\shortstack{Accuracy \\ Baseline=0.554707}} & \textbf{Precision} & \textbf{Recall} & \textbf{F1 score}\\
        \hline
        \hline
        AAD-LLM & 0.584337 & 0.467391 & 0.682540 & 0.555839 \\
        \hline
        RAAD-LLM & 0.715861 & 0.628376 & 0.885714 & 0.735114 \\
        \hline
        RAAD-LLMv2 & 0.683630 & 0.608254 & 0.813333 & 0.695995 \\
        \hline
    \end{tabular}
    \vspace{4mm}
    \caption{Average evaluation metrics over multiple model runs. The baseline model is one that predicts every observation to belong to the majority class. The RAG pipeline for both RAAD-LLM and RAAD-LLMv2 integrate a CSV-based knowledge base to dynamically retrieve contextually relevant information for z-score comparisons, allowing for responses that reflect either exact matches for input values or the closest matches when exact values are not found. RAAD-LLMv2 integrates LlamaIndex for seamless retrieval of relevant domain knowledge from the vector store. Unlike RAAD-LLM, RAAD-LLMv2 adds only the retrieved content to the prompt before being fed forward through the frozen LLM.} \label{table:tab_results1}
    \end{center}
\end{table}


\begin{table*}[!t]
    \begin{center}
    \begin{tabular}{| c | c | c | c | c | c | c | c |}
    \hline
    \textbf{Algorithm} & \textbf{F1} & \textbf{FAR, \%} & \textbf{MAR, \%} & \textbf{No Training or Fine-tuning} & \textbf{Multimodal} \\
    \hline
    \hline
    Perfect detector & 1 & 0 & 0 & & \\
    \hline
    \textbf{RAAD-LLM} & \textbf{0.74} & \textbf{42.05} & \textbf{11.43} & \textbf{yes} & \textbf{yes} \\
    \hline
    LSTMCaps \cite{Elhalwagy_2022} & 0.74 & 21.5 & 18.74 & no & no \\
    \hline
    MSET \cite{mset} & 0.73 & 20.82 & 20.08 & no & no \\
    \hline
    LSTMCapsV2 \cite{Elhalwagy_2022} & 0.71 & 14.51 & 30.59 & no & no \\
    \hline
    \textbf{RAAD-LLMv2} & \textbf{0.70} & \textbf{42.05} & \textbf{18.67} & \textbf{yes} & \textbf{yes} \\
    \hline
    MSCRED \cite{Zhang_Song_Chen_Feng_Lumezanu_Cheng_Ni_Zong_Chen_Chawla_2019} & 0.70 & 16.2 & 30.87 & no & no \\
    \hline
    Vanilla LSTM \cite{filonov2016multivariateindustrialtimeseries} & 0.67 & 15.42 & 36.02 & no & no \\
    \hline
    Conv-AE \cite{conv_ae}	& 0.66 & 5.58 & 46.05 & no & no \\
    \hline
    LSTM-AE \cite{lstm_ae} & 0.65 & 14.59 & 39.42 & no & no \\
    \hline
    \textbf{AAD-LLM} & \textbf{0.56} & \textbf{47.6} & \textbf{31.7} & \textbf{yes} & \textbf{yes} \\
    \hline
    LSTM-VAE \cite{Bowman2015GeneratingSF} & 0.56 & 9.2 & 54.81 & no & no \\
    \hline
    Vanilla AE \cite{Chen2017OutlierDW} & 0.45 & 7.55 & 66.57 & no & no \\
    \hline
    Isolation forest \cite{4781136} & 0.4 & 6.86 & 72.09 & no & no \\
    \hline
    Null detector & 0 & 100 & 100 & & \\
    \hline
    \end{tabular}
    \caption{Best outlier detection scores for each anomaly detection method implemented on the SKAB dataset, sorted by F1 score \cite{Elhalwagy_2022}. A selection of NNs and ML based fault detection methods were chosen to compare on the benchmarks. RAAD-LLM and RAAD-LLMv2 metrics are averaged over multiple model runs. Multimodality allows for the enriching of input series data with semantics to enable more collaborative decision-making between the model and plant operators. For this work, multimodality refers to a model being optimized to detect anomalies across both time-series data and text. A model that requires no training or fine-tuning on the data it is applied to is considered transferable with zero-shot capabilities. Unlike all other methods, AAD-LLM, RAAD-LLM, and RAAD-LLMv2 are not trained or fine-tuned on the dataset they are applied to and are multimodal without requiring any additional strategies.} 
    \label{table:tab_results2}
    \end{center}
\end{table*}

To assess the performance of the frameworks, we applied RAAD-LLM and RAAD-LLMv2 to both the SKAB and use-case datasets. Evaluation metrics include accuracy, precision, recall, and F1-score, with a particular focus on the model's ability to reduce false positives and improve anomaly detection rates when compared to the original AAD-LLM. 

The brief results are shown in Table \ref{table:tab_results1}. For the use-case dataset, RAAD-LLM achieved an accuracy of $89.1 \pm 1.5\%$, which is a significant improvement over the baseline model. This indicates that the model is indeed useful. Furthermore, RAAD-LLM's precision of $96.7 \pm 0.04\%$, recall of $88.2 \pm 2.1\%$ and F1 score of $92.2 \pm 1.2\%$ are all notable improvements over the previous architecture. For the SKAB dataset, RAAD-LLM achieved an accuracy of $72.0 \pm 0.4\%$, F1 score of $73.5 \pm 0.7\%$, FAR of $42.1 \pm 0.9\%$, and MAR of $11.4 \pm2.1\%$. As with the use-case dataset, all evaluation metrics for the SKAB dataset show a significant improvement over the previous architecture.

\autoref{fig:fig_metrics} shows average performance metrics and their variability over multiple model runs for RAAD-LLM versus RAAD-LLMv2. While RAAD-LLMv2 injects only relevant information and eliminates the need for manual context restructuring, it exhibited lower performance metrics for both datasets when compared to RAAD-LLM. This performance trade-off highlights the challenges posed by dynamic knowledge retrieval in the RAAD-LLMv2 framework. Although RAAD-LLM is shown to be highly effective in controlled scenarios where manual context restructuring is feasible, RAAD-LLMv2 is a more scalable alternative for real-world scenarios requiring automated domain knowledge retrieval. These findings reveal opportunities for further optimization to improve RAAD-LLMv2's overall performance.

\begin{figure}
    \includegraphics[width=0.5\textwidth]{images/uc-metrics.png}
    \vspace{6mm}
    \caption{Average performance metrics and their variability over multiple model runs for RAAD-LLM versus RAAD-LLMv2. RAAD-LLMv2 exhibited lower performance for all metrics compared to RAAD-LLM for both datasets.}
    \label{fig:fig_metrics}
\end{figure}

\autoref{table:tab_results2} summarizes the scores for algorithms on $3$ application benchmarks using the SKAB dataset, sorted by F1 score. For F1 score, bigger is better. For both FAR and MAR, less is better. While our previous architecture ranked $8^{th}$ among all NN and ML based methods, RAAD-LLM and RAAD-LLMv2 ranked $1^{st}$ and $4^{th}$, respectively in F1 score. Although, both RAAD-LLM and RAAD-LLMv2 ranked last in FAR, they ranked $1^{st}$ and $2^{nd}$, respectively in MAR. In industrial applications where there is potential for severe safety implications and the risk of catastrophic failure, the MAR is generally considered more important and is often prioritized. Effective anomaly detection systems should strive to minimize both FAR and MAR, but special attention should be given to ensuring that real anomalies are not overlooked, as the consequences of such oversights can far outweigh the inconveniences posed by false alarms.

The integration of the RAG component into the RAAD-LLM and RAAD-LLMv2 frameworks has led to marked improvements in anomaly detection performance compared to the previous AAD-LLM architecture. Results indicate that RAG enhances the model's performance in detecting anomalies within time series data. Our findings affirm the efficacy of RAG in augmenting the capabilities of LLMs in PdM applications. With RAAD-LLM outperforming all presented fault detection methods, repurposing LLMs with RAG integration is shown effective in detecting anomalies in time series data accurately. Overall, our findings support the use of LLMs for anomaly detection for the PdM use-case, underlining their capability and potential in handling challenges in time series anomaly detection in data-constrained industrial applications. This work significantly advances anomaly detection methodologies, potentially leading to a paradigm shift in how anomaly detection is implemented across various industries.


